Inductive-data-type Systems

In a previous work ("Abstract Data Type Systems", TCS 173(2), 1997), the last two authors presented a combined language made of a (strongly normalizing) algebraic rewrite system and a typed lambda-calculus enriched by pattern-matching definitions following a certain format, called the "General Schema", which generalizes the usual recursor definitions for natural numbers and similar "basic inductive types". This combined language was shown to be strongly normalizing. The purpose of this paper is to reformulate and extend the General Schema in order to make it easily extensible, to capture a more general class of inductive types, called "strictly positive", and to ease the strong normalization proof of the resulting system. This result provides a computation model for the combination of an algebraic specification language based on abstract data types and of a strongly typed functional language with strictly positive inductive types.

==> interpretation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% function interpretation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\append{Function interpretation}

\newcommand{\si}{{s_i}}
\newcommand{\ns}{_{\not\ts}}

In this appendix, we define the function interpretations $\Phi_f$ and
the orderings $\ge_f$ used in Lemma~\ref{lem-comp-hofs} and prove that
they satisfied the properties given in Definition~\ref{def-interpret}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% definition
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Definition}

Since the interpretation must be compatible with the reduction
relation, the idea is to interpret a term by its reducts.  Besides,
since the comparisons are done with critical subterms at inductive
positions, we can erase all subterms that are not $\ts$-positive. For
these two ideas to be compatible, we take into account only reducts
obtained via rewrites of $\ts$-positive subterms.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% positive reductions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{defn}[Positive reductions]
  We will denote by $u \tge_\ts v$ the fact that $v$ is an
  $\ts$-positive subterm of $u$ (see Definition~\ref{def-critical}).
  
  Given an inductive type $\ts$, we define the {\em $\ts$-rewrite
    relation} as being the restriction of the IDTS rewrite relation to
  $\ts$-positive terms. The {\em $\ts$-reduction relation} is the
  reflexive and transitive closure of the $\ts$-rewrite relation. A
  term is in {\em $\ts$-normal form} if it cannot be $\ts$-reduced.
  Given a strongly normalizable term $u$, we denote by $R_\ts(u)$ the
  least set containing $u$ and stable by $\ts$-reduction.
  
  We define the {\em co-$\ts$-rewrite relation} by: $u \a\ns^p u'$ iff
  $u$ reduces to $u'$ at position $p$ and $u$ is not $\ts$-reducible
  at position $p$.
\end{defn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% erasing function
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{defn}[Erasing function]
  For each type $t$, we assume given a function symbol $\bot_t$ of
  arity 0 and type $t$. Given an inductive type $\ts \in \cI$, the
  {\em $\ts$-erasing function} $\Psi_\ts$ is defined as follows:

\begin{itemize}
\item $\Psi_\ts(u) = \bot_t$ if $u$ is of type $t$ and $\ts$ does not
  occur positively in $t$ (i.e. it is not an $\ts$-positive term).
\end{itemize}

Otherwise, $\Psi_\ts(u)$ is defined by case on $u$:

\begin{itemize}
\item $\Psi_\ts(x) = x$,
\item $\Psi_\ts(f(u_1, \ldots, u_n)) = f(\Psi_\ts(u_1), \ldots,
  \Psi_\ts(u_n))$,
\item $\Psi_\ts(\l x. u) = \l x.  \Psi_\ts(u)$,
\item $\Psi_\ts((u ~v)) = (\Psi_\ts(u) ~\Psi_\ts(v))$.
\end{itemize}
\end{defn}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% function interpretation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{defn}[Function interpretation]
\label{def-rec-call-inter}
Given a function symbol $f \in \cF_{s_1, \ldots, s_n, s}$, we define
its {\em function interpretation} $\Phi_f$ on strongly normalizable
arguments of $f$ as follows:

\begin{itemize}
\item $\Phi_f(u_1, \ldots, u_n) = (\Phi_f^{1}(u_1), \ldots,
  \Phi_f^{n}(u_n))$,
\item $\Phi_f^i(u_i) =
  \left\{
    \begin{array}{l@{~~\mr{if}~~}l}
    \{ u_i \} & i \notin Ind(f)\\
    \h{\Psi_\si}(R_\si(\chi_\si(u_i))) & i \in Ind(f),\\
    \end{array}
  \right.$
\end{itemize}

where $\h{\Psi_\si}$ is the extension of $\Psi_\si$ on multisets. Its
associated ordering is $\ge_f \,= ((\a \cup ~\tgt)\mul)\stat$.
\end{defn}

It is not difficult to see that $\ge_f \,=\, \ge_g$ whenever $f =_\cF
g$ since, in this case, we assume that $stat_f = stat_g$. Furthermore,
$>_f$ is clearly well-founded on strongly normalizable arguments of
$f$. Before to prove the stability and the $\a$-compatibility, we
establish some properties of $R_\ts$, $\Psi_\ts$ and $\h{\Psi_\ts}$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% properties
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Properties}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% $R_\ts$ properties
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}[$R_\ts$ properties]
Assume that $u$ and $v$ are two strongly normalizable terms.

\begin{enumerate}
\item If $u \tgt_\ts v$ then $R_\ts(u) ~(\tgt_\ts)\mul ~R_\ts(v)$.
\item If $u \a_\ts v$ then $R_\ts(u) \sge R_\ts(v)$.
\item If $u \a\ns v$ then $R_\ts(u) ~(\a\ns)\mul ~R_\ts(v)$.
\end{enumerate}
\end{lem}

\begin{pf}
\begin{enumerate}
\item Suppose that $v = u|_p$. Let $v' \in R_\ts(v)$.  Since $u
  \tgt_\ts v$, each superterm of $v$ in $u$ is an $\ts$-positive term.
  Hence, $u[v']_p \in R_\ts(u)$ and $u[v']_p \tgt_\ts v'$.
\item Immediate.
\item Let $v' \in R_\ts(v)$ and $p \in Pos(u)$ be a position such that
  $u \a\ns^p v$. If $u$ is not $\ts$-positive then, by subject
  reduction, $v$ is not $\ts$-positive either. Hence, $R_\ts(u) = \{ u
  \} ~(\a\ns)\mul ~R_\ts(v) = \{ v \}$. Otherwise, there exists a
  superterm $w = u|_{p_1} \;(p = p_1 p_2)$ of $u|_p$ which is not
  $\ts$-positive but whose superterms are $\ts$-positive. Then, $w
  \a\ns^{p_2} w' = v|_{p_1}$ and $v = u[w']_{p_1}$. Now, let $v' \in
  R_\ts(v)$. The $\ts$-reductions from $v$ to $v'$ can be also carried
  out on $u$. Therefore there is a term $u' \in R_\ts(u)$ such that
  $u' \a\ns^* v'$. (Take the term obtained by replacing in $v'$ all
  the occurrences of $w'$ by $w$.)
\end{enumerate}
\end{pf}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% $\Psi_\si$ properties
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}[$\Psi_\ts$ properties]
\hfill
\begin{enumerate}
\item $\Psi_\ts$ preserves types: if $u \in \L^t$ then $\Psi_\ts(u)
  \in \L^t$.
\item If $u \tgt_\ts v$ then $\Psi_\ts(u) \tgt_\ts \Psi_\ts(v)$.
\item If $u \a\ns v$ then $\Psi_\ts(u) = \Psi_\ts(v)$.
\end{enumerate}
\end{lem}

\begin{pf}
\begin{enumerate}
\item Immediate.
\item Suppose that $v = u|_p$. Since each superterm of $v$ in $u$ has
  a type in which $\ts$ occurs positively, $\Psi_\ts(u) =
  \Psi_\ts(u)[\Psi_\ts(v)]_p$. Since $\Psi_\ts$ preserves typing,
  $\Psi_\ts(u) \tgt_\ts \Psi_\ts(v)$.
\item Suppose that $u\a\ns^p v$. If $u$ is not $\ts$-positive then
  $\Psi_\ts(u) = \Psi_\ts(v) = \bot_t$ where $t$ is the type of $u$.
  Otherwise, $v$ has a superterm $w = u|_{p_1} \;(p = p_1 p_2)$ in $u$
  which is not $\ts$-positive but whose superterms are $\ts$-positive.
  Hence, $\Psi_\ts(u) = \Psi_\ts(u)[\bot_t]_{p_1}$ where $t$ is the
  type of $w$. Since $w \a\ns^{p_2} w' = v|_{p_1}$, $v = u[w']_{p_1}$
  and $w'$ is not $\ts$-positive, $\Psi_\ts(v) = \Psi_\ts(u)$.
\end{enumerate}
\end{pf}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% $\h{\Psi_\si}$ properties
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{lem}[$\h{\Psi_\ts}$ properties]
Assume that $u$ and $v$ are two strongly normalizable terms.

\begin{enumerate}
\item If $u \tgt_\ts v$ then $\h{\Psi_\ts}(R_\ts(u)) ~(\tgt_\ts)\mul
  ~\h{\Psi_\ts}(R_\ts(v))$.
\item If $u \a v$ then $\h{\Psi_\ts}(R_\ts(u)) ~(\a\ns)\mul
  ~\h{\Psi_\ts}(R_\ts(v))$.
\end{enumerate}
\end{lem}

\begin{pf}
  By composing the properties of $R_\ts$ and $\Psi_\ts$.
\end{pf}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% stability of the interpretation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Stability}

\begin{lem}[Stability]
\label{lem-stab}
Let $\vec{u}$ be arguments of $f$ and $\vec{v}$ be arguments of $g
=_\cF f$. Let $\t$ be a substitution such that the terms in
$\vec{u}\t$ and $\vec{v}\t$ are strongly normalizable. If
$FV(\phi_g(\vec{v})) \sle FV(\vec{u})$ and $\phi_f(\vec{u}) = \vec{u}
~\tgt\stat \phi_g(\vec{v})$ then $\Phi_f(\vec{u}\t) >_f
\Phi_g(\vec{v}\t)$.
\end{lem}

\begin{pf}
  Let us assume that $\vec{u} ~\tgt\stat \phi_g(\vec{v})$ results from
  the comparison between $u_i$ and $\phi_g^j(v_j)$. There are two
  cases:

\begin{enumerate}
\item If $i \in Ind(f)$ then $j = i$ since, by definition of status,
  inductive positions are lexicographic. Hence, $\phi_f^i(v_i) =
  \chi_\si(v_i)$, $\Phi_f^i(u_i\t) =
  \h{\Psi_\si}(R_\si(\chi_\si(u_i\t)))$ and $\Phi_f^i(v_i\t) =
  \h{\Psi_\si}( R_\si(\chi_\si(v_i\t)))$. By definition of the General
  Schema, $\chi_\si(u_i) = u_i \tgt_\si \chi_\si(v_i)$.  Hence
  $\chi_\si(u_i)$ cannot be a variable and $\chi_\si(u_i\t) =
  \chi_\si(u_i)\t = u_i\t$. Besides, since $FV(\chi_\si(v_i)) \sle
  FV(\vec{u})$, $u_i\t ~\tgt_\si ~\chi_\si(v_i)\t ~\tge_\si \\
  ~\chi_\si(v_i\t)$. By property of $\h{\Psi_\si}$,
  $\h{\Psi_\si}(R_\si(\chi_\si(u_i\t))) ~(\tgt_\si)\mul
  ~\h{\Psi_\si}(R_\si(\chi_\si(v_i\t)))$.
  
\item If $i \notin Ind(f)$ then $j \notin Ind(f)$, $\phi_f^j(v_j) =
  v_j$, $\Phi_f^i(u_i\t) = \{ u_i\t \}$ and $\Phi_f^j(u_j\t) = \{
  u_j\t \}$. Since $FV(v_j) \sle FV(\vec{u})$, $u_i\t ~\tgt ~v_j\t$
  and $\Phi_f^i(u_i\t) ~\tgt\mul \Phi_f^j(v_j\t)$.
\end{enumerate}
\end{pf}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% compatibility of the interpretation
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{$\a$-Compatibility}

\begin{lem}[Compatibility]
\label{lem-comp}
Assume that $\vec{u}$ and $\vec{u'}$ are strongly normalizable
arguments of $f$ such that $\vec{u} \a\lex \vec{u'}$. Then,
$\Phi_f(\vec{u}) \ge_f \Phi_f(\vec{u'})$.
\end{lem}

\begin{pf}
  We prove the lemma for one rewrite. Suppose that $u_i \a u'_i$. We
  distinguish two cases:

\begin{enumerate}
\item If $i \notin Ind(f)$ then $\Phi_f^i(u_i) = \{ u_i \}$ and
  $\Phi_f^i(u'_i) = \{ u'_i \}$. Since $u_i \a u'_i$, $\Phi_f^i(u_i)
  ~\a\mul ~\Phi_f^i(u'_i)$.
  
\item If $i \in Ind(f)$ then $\Phi_f^i(u_i) =
  \h{\Psi_\si}(R_\si(\chi_\si(u_i)))$ and $\Phi_f^i(u'_i) = \hfill\\
  \h{\Psi_\si}(R_\si(\chi_\si(u'_i)))$. Let us write $u_i = b_1 \ldots
  b_p \;(p \ge 1)$ such that $b_1$ is not an application and suppose
  that $\chi_\si(u_i) = b_1 \ldots b_k \;(1 \le k \le p)$. Then, we
  distinguish four subcases:

  \begin{enumerate}
  \item If $u_i$ is reduced in $b_j \;(k+1 \le j \le p)$ then, by
    subject reduction, $\chi_\si(u'_i) = \chi_\si(u_i)$.

  \item If $u_i$ is reduced in $b_j \;(1 \le j \le k, k \ge 2)$ then
    $\chi_\si(u_i) \a \chi_\si(u'_i)$ and, by property of
    $\h{\Psi_\si}$, $\h{\Psi_\si}(R_\si(\chi_\si(u_i))) ~(\a\ns)\mul
    ~\h{\Psi_\si}(R_\si(\chi_\si(u'_i)))$.
    
  \item If $u_i$ is reduced in $b_1$ and $k=1$ then $\chi_\si(u_i) \a
    b'_1$ and $\chi_\si(u'_i) = \chi_\si(b'_1)$. By property of
    $\h{\Psi_\si}$, $\h{\Psi_\si}(R_\si(\chi_\si(u_i))) ~(\a\ns)\mul
    ~\h{\Psi_\si}(R_\si(b'_1)) \\ ~(\tgt_\si)\mul
    ~\h{\Psi_\si}(R_\si(\chi_\si(b'_1)))$.
    
  \item Suppose now that $p\ge 2$, $b_1 = \l x. c$ and $u'_i = c \{ x
    \to b_2 \} \,b_3 \ldots b_p$. There are three subcases:

    \begin{enumerate}
    \item If $k\ge 3$ then $\chi_\si(u_i) \a \chi_\si(u'_i)$. By
      property of $\h{\Psi_\si}$,\\
      $\h{\Psi_\si}(R_\si(\chi_\si(u_i))) ~(\a\ns)\mul
      ~\h{\Psi_\si}(R_\si(\chi_\si(u'_i)))$.
    
    \item If $k=2$ then $\chi_\si(u'_i) = \chi_\si(c \{ x \to b_2
      \})$. By property of $\h{\Psi_\si}$,
      $\h{\Psi_\si}(R_\si(\chi_\si(u_i))) ~(\a\ns)\mul
      ~\h{\Psi_\si}(R_\si( c \{ x \to b_2 \})) ~(\tgt_\si)\mul \\
      ~R_\si(\chi_\si(u'_i))$.
    
    \item If $k=1$ then, by definition of $s_i$-critical subterm,
      $s_i$ occurs positively in the type $t$ of $\l x. c$ and in the
      type $t'$ of $(\l x. c ~b_2)$. Let $t_2$ be the type of $b_2$.
      Then, $t= t_2 \a t'$ and $s_i$ does not occur or occurs
      negatively in $t_2$. Therefore, $c\neq x$, $\chi_\si(u'_i) =
      \chi_\si(c) \{ x \to b_2 \}$, $R_\si(\chi_\si(u'_i)) = \{ d \{ x
      \to b_2 \} ~|~ d \in R_\si(\chi_\si(c))\}$ and
      $\h{\Psi_\si}(R_\si(\chi_\si(u'_i))) =
      \h{\Psi_\si}(R_\si(\chi_\si(c)))$. Besides,\\
      $\h{\Psi_\si}(R_\si(\chi_\si(u_i))) = \{ \l x.  c' ~|~ c' \in
      \h{\Psi_\si}(R_\si(c))\} ~\tgt\mul \h{\Psi_\si}(R_\si(c))\\
      ~(\tgt_\si)\mul ~\h{\Psi_\si}(R_\si(\chi_\si(c)))$.
    \end{enumerate}

  \end{enumerate}

\end{enumerate}
\end{pf}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 


==> strict.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% recursors for strictly positive types
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\append{Recursors for strictly positive types}

Assume that $\ts$ is a strictly positive inductive type (non-mutually
defined) with $n$ constructors $C_1, \ldots, C_n$ such that $\tau(C_i)
= s_{i,1} \a \ldots \a s_{i,n_i} \a \ts$ and $s_{i,j} = s_{i,j,1} \a
\ldots \a s_{i,j,n_{i,j}} \a \mt{t}_{i,j}$. Then, $\mt{t}_{i,j}
\le_\cF \ts$ and $\ts$ occurs in no $s_{i,j,k}$.

Given an arbitrary type $t$, the recursor for $\ts$ of output type $t$
is a function symbol $srec_t$ of arity $n + 1$ and type $t_1 \a \ldots
\a t_n \a \ts \a t$ where $t_i = s_{i,1} \a \ldots \a s_{i,n_i} \a
s_{i,1}' \a \ldots \a s_{i,n_i}' \a t$ and, for any type $s$, $s'$
denotes the type $s$ in which each occurrence of $\ts$ has been
replaced by $t$. Then, the rewrite rules defining $srec_t$ are the
following:

\begin{rewc}
$srec_t(Y_1, \ldots, Y_n, C_i(x_1, \ldots, x_{n_i}))$
& $(Y_i ~x_1 \ldots x_{n_i} ~x_1' \ldots x_{n_i}')$\\
\end{rewc}

where $x_j' =
  \left\{
    \begin{array}{l}
    x_j ~~\mr{if}~ ~\mt{t}_{i,j} <_\cI \ts\\
    \l z_1 \ldots z_{n_{i,j}}. srec_t(Y_1, \ldots, Y_n, (x_j
           ~z_1 \ldots z_{n_{i,j}})) ~~\mr{if} ~\mt{t}_{i,j} = \ts\\
    \end{array}
  \right.$

\begin{lem}
  The recursor rules for strictly positive inductive types follow the
  General Schema.
\end{lem}

\begin{pf}
  We prove that the right-hand side $(Y_i ~x_1 ~... ~x_{n_i} ~x_1'
  ~... ~x_{n_i}')$ belongs to the computable closure of the left-hand
  side $srec_t(Y_1, ..., Y_n, C_i(x_1, ..., x_{n_i}))$, by taking
  $stat_{srec_t} = lex(mul(y_{n+1}))$ and $Ind(srec_t) = \{ n+1 \}$.
  
  The variables $Y_1, \ldots, Y_n$ and $x_1, \ldots, x_{n_i}$ are
  accessible since the formers are left-hand side arguments of
  $srec_t$, while the latters are arguments of the constructor-headed
  term $C_i(x_1, \ldots, x_{n_i})$ which is an argument of $srec_t$.
  The $\ts$-critical subterm of $(x_j ~z_1 \ldots z_{n_{i,j}})$ is
  $x_j$ since it is the smallest $\ts$-positive subterm of $(x_j ~z_1
  \ldots z_{n_{i,j}})$ (its type is $s_{i,j} = s_{i,j,1} \a \ldots \a
  s_{i,j,n_{i,j}} \a \ts$). Hence, the recursive calls $srec_t(Y_1,
  \ldots, Y_n, (x_j ~z_1 \ldots z_{n_{i,j}}))$ belong to the
  computable closure since $x_j$ is a strict subterm of $C_i(x_1,
  \ldots, x_{n_i})$. By using the computability preserving operations
  of the computable closure, it follows that the whole right-hand side
  belongs to the computable closure.
\end{pf}




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

